Collaboration in Immersive Environments: Challenges and Solutions

Virtual Reality (VR) and Augmented Reality (AR) tools have been applied in all engineering fields in order to avoid the use of physical prototypes, to train in high-risk situations, and to interpret real or simulated results. In order to complete a shared task or assign tasks to the agents in such immersive environments, collaboration or Shared Cooperative Activities are a necessity. Collaboration in immersive environments is an emerging field of research that aims to study and enhance the ways in which people interact and work together in Virtual and Augmented Reality settings. Collaboration in immersive environments is a complex process that involves different factors such as communication, coordination, and social presence. This paper provides an overview of the current state of research on collaboration in immersive environments. It discusses the different types of immersive environments, including VR and AR, and the different forms of collaboration that can occur in these environments. The paper also highlights the challenges and limitations of collaboration in immersive environments, such as the lack of physical cues, cost and usability and the need for further research in this area. Overall, collaboration in immersive environments is a promising field with a wide range of potential applications, from education to industry, and it can benefit both individuals and groups by enhancing their ability to work together effectively.

==> Sections/ToDoList.tex <==

To Dos:

By Mar 31
- Finish Application section
- Add references

By Apr 5
- Evaluate all finished sections for any changes including add/edit/remove
- Design related figures
- Design related tables/charts taxonomy 

By Apr 15
- Finish the presentation PPT

---------------
Presentation ToDos:
Around 25 pages

Sections:

- My Introduction
- My work Introduction
- Why

- Survey Introduction
Subsections

- Challenges
Subsections

- Solutions
Subsections

- Applications
Subsections

- Conclusion
Subsections


---------------

Finalized sections:

- Abstract -     Done
- Introduction - Done
- Challenges -   Done
- Methodology -  Done
- Applications - Done
- Conclusion -   Done


---------------
Any related conference to apply?

QE committee ?

KRS : OK
Alexia : OK
Wenwen : OK

---------------

Presentation Schedule - Excel file

---------------
CPT
Will send a request

